Tell Me Where to Go: A Composable Framework for Context-Aware Embodied Robot Navigation

Humans have the remarkable ability to navigate through unfamiliar environments by solely relying on our prior knowledge and descriptions of the environment. For robots to perform the same type of navigation, they need to be able to associate natural language descriptions with their associated physical environment with a limited amount of prior knowledge. Recently, Large Language Models (LLMs) have been able to reason over billions of parameters and utilize them in multi-modal chat-based natural language responses. However, LLMs lack real-world awareness and their outputs are not always predictable. In this work, we develop NavCon, a low-bandwidth framework that solves this lack of real-world generalization by creating an intermediate layer between an LLM and a robot navigation framework in the form of Python code. Our intermediate shoehorns the vast prior knowledge inherent in an LLM model into a series of input and output API instructions that a mobile robot can understand. We evaluate our method across four different environments and command classes on a mobile robot and highlight our NavCon's ability to interpret contextual commands.

==> introduction.tex <==
\section{Introduction}
\label{sec:intro}

As humans, we are able to intelligently navigate in a new environment such as a town or a building based on a cognitive map generated by our prior knowledge \cite{mcnamara1989subjective}. Mobile robots have been deployed in a variety of tasks ranging from vacuums navigating around a home \cite{tellex2020robots} to quadrupeds exploring unknown environments within the context of search and rescue \cite{DARPA2022, biggie2023flexible}. In order to successfully navigate, these systems typically rely on metric-based planners and localization systems which are non-intuitive for humans. A much more efficient method of directing these systems would be to use natural language instructions.

Associating natural language to an embodied agent requires grounding utterances to the physical world in which the robot operates within. Various approaches have been used to associate language to the physical domain ranging from probabilistic graph based structures \cite{tellex2011understanding,howard2014natural,kollar2010toward} to end to end learning based methods \cite{driess2023palm}. Graph based approaches have shown a lot of promise but their generalizability is limited to a fixed training corpus which needs manual annotation. Recently large language models (LLMs) have proven to be incredibly adept at reasoning over large amounts of unsupervised training data \cite{floridi2020gpt, touvron2023llama} using transformer based backends \cite{vaswani2017attention}. We wish to leverage this vast knowledge base on an embodied agent while ensuring a degree of explainability.

While the beauty of LLMs is their ability to generalize, they also have no concept of truth or the physical world. These models can produce inherently wrong outputs without constraints which produces enormous safety challenges when associating them with a physical system. As such we propose using a intermediate layer which is able to extract the necessary prior information required for navigation tasks from an LLM and constrain it to outputs that can be acted on by traditional robotic navigation planners. We do this in the form of generated Python code from GPT-4 \hjb{need to cite} using a fixed API in a similar fashion to \cite{suris2023vipergpt}. The fixed API ensures the robot can act upon the information extracted from the LLM while providing a degree of explainability. We are able to see why certain navigation commands fail and more importantly we show that we can explain to non robotics expert the failure modes.


